Differentiable Cutting-plane Layers for Mixed-integer Linear Optimization

We consider the problem of solving a family of parametric mixed-integer linear optimization problems where some entries in the input data change. We introduce the concept of cutting-plane layer (CPL), i.e., a differentiable cutting-plane generator mapping the problem data and previous iterates to cutting planes. We propose a CPL implementation to generate split cuts, and by combining several CPLs, we devise a differentiable cutting-plane algorithm that exploits the repeated nature of parametric instances. In an offline phase, we train our algorithm by updating the internal parameters controlling the CPLs, thus altering cut generation. Once trained, our algorithm computes, with predictable execution times and a fixed number of cuts, solutions with low integrality gaps. Preliminary computational tests show that our algorithm generalizes on unseen instances and captures underlying parametric structures.

==> headers/definitions.tex <==
% Define new boolean flag
\newbool{boldSymbols}

% Set to true to make symbols bold
% \setbool{boldSymbols}{true}

% Set to false to make symbols not bold
\setbool{boldSymbols}{false}

% Sets
\newcommand{\maxi}{\text{maximize}}
\newcommand{\mini}{\text{minimize}}
\newcommand{\st}{\text{subject to}}
\newcommand{\X}[1]{ \ifbool{boldSymbols}{\mathcal{X}}{X}^{ #1 }} 
\newcommand{\ones}{\mathbf 1}
\newcommand{\R}{\ifbool{boldSymbols}{\mathbb{R}}{\mathbf{R}}}
\newcommand{\Z}{\ifbool{boldSymbols}{\mathbb{Z}}{\mathbf{Z}}}
\newcommand{\Q}{\ifbool{boldSymbols}{\mathbb{Q}}{\mathbf{Q}}}
\newcommand{\NPhard}{\mbox{$\mathcal{NP}$-hard}\xspace}  
\newcommand{\identity}{\ifbool{boldSymbols}{\mathbf{I}}{I}}
\newcommand{\diag}{\operatorname{\bf diag}}
\newcommand{\Expect}{\operatorname{\bf E{}}}
\newcommand{\conv}{\operatorname{\bf conv}}
\newcommand{\integer}{\operatorname{int}}
\newcommand{\rec}{\operatorname{rec}}
\newcommand{\lin}{\operatorname{lin}}
\newcommand{\bd}{\operatorname{bd}}
\newcommand{\cl}{\operatorname{cl}}
\newcommand{\proj}{\operatorname{proj}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\cone}{\operatorname{cone}}
\newcommand{\epi}{\operatorname{\bf epi}} % epigraph
\newcommand{\Vol}{\operatorname{\bf vol}}
\newcommand{\dom}{\operatorname{\bf dom}} % domain

\newcommand{\sign}{\operatorname{\bf sign}}
\newcommand{\round}{\operatorname{\bf round}}
\newcommand{\define}{\coloneqq}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}

% Add Clevref names
\crefname{line}{Line}{Lines}
\crefname{lemma}{Lemma}{Lemmata}
\crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\crefname{algorithm}{Algorithm}{Algorithms}
\crefname{equation}{}{}
\crefname{definition}{Definition}{Definition}
\crefname{claim}{Claim}{Claim}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{remark}{Remark}{Remarks}
\crefname{example}{Example}{Examples}
\crefname{figure}{Figure}{Figures}
\crefname{section}{Section}{Sections}
\crefname{table}{Table}{Tables}


% Acronyms
\usepackage[xindy, acronyms, nowarn]{glossaries}   % Glossaries and Acronyms
\glsdisablehyper
\makeglossaries
% Acronyms
\newglossaryentry{MIP}
{
  name={MIP},
  plural={MIPs},
  description={mixed-integer optimzation problem},
  first={mixed-integer optimization problem (\glsentrytext{MIP})},
  descriptionplural={mixed-integer optimzation problem},
  firstplural={mixed-integer optimization problems (\glsentryplural{MIP})}
}
\newglossaryentry{CPL}
{
  name={CPL},
  plural={CPLs},
  description={cutting-plane layer},
  first={cutting-plane layer (\glsentrytext{CPL})},
  descriptionplural={cutting-plane layers},
  firstplural={cutting-plane layers (\glsentryplural{CPL})}
}

\newglossaryentry{CGP}
{
  name={CGP},
  plural={CGPs},
  description={cut-generating program},
  first={cut-generating program (\glsentrytext{CGP})},
  descriptionplural={cut-generating program},
  firstplural={cut-generating programs (\glsentryplural{CGP})}
}
\newglossaryentry{CGLP}
{
  name={CGLP},
  plural={CGLPs},
  description={cut-generating linear program},
  first={cut-generating linear program (\glsentrytext{CGLP})},
  descriptionplural={cut-generating linear programs},
  firstplural={cut-generating linear programs (\glsentryplural{CGLP})}
}
\newglossaryentry{RNN}
{
    name={RNN},
    description={recurrent neural network}
}


\newcommand{\parameters}{\ifbool{boldSymbols}{\boldsymbol{\theta}}{\theta}}
\newcommand{\cutparameters}{\ifbool{boldSymbols}{\boldsymbol{\sigma}}{\sigma}}
\newcommand{\rnnparameters}{\ifbool{boldSymbols}{\boldsymbol{\rho}}{\rho}}
\newcommand{\variables}{\ifbool{boldSymbols}{\mathbf{x}}{x}}
\newcommand{\numintegers}{n_i}
\newcommand{\integeridx}{\mathcal{I}}
\newcommand{\numcontinuous}{n_c}
\newcommand{\numconstraints}{m}
\newcommand{\numvars}{n}
\newcommand{\numtraining}{N}
\newcommand{\parameterset}{\Theta}
\newcommand{\probA}{\ifbool{boldSymbols}{\mathbf{A}}{A}(\parameters)}
  \newcommand{\probc}{\ifbool{boldSymbols}{\mathbf{c}}{c}(\parameters)}
  \newcommand{\probb}{\ifbool{boldSymbols}{\mathbf{b}}{b}(\parameters)}
\newcommand{\probregion}{X(\parameters)}
\newcommand{\probrelaxregion}{\tilde{X}(\parameters)}
\newcommand{\probexactregion}{\conv(\probregion)}
\newcommand{\optimal}{\ifbool{boldSymbols}{\mathbf{x}}{x}^\star(\parameters)}
\newcommand{\relaxsolution}[1]{\ifbool{boldSymbols}{\mathbf{x}}{x}^{#1}(\parameters)}
\newcommand{\toseparate}{\bar{\ifbool{boldSymbols}{\mathbf{x}}{x}}}
\newcommand{\relaxobjective}[1][]{z^{ #1 }(\parameters)}
\newcommand{\optimalobjective}{z^\star(\parameters)}
\newcommand{\cutsRHS}[1][]{\ifbool{boldSymbols}{\mathbf{h}}{h}^{#1}(\parameters)}
\newcommand{\cutsLHS}[1][]{\ifbool{boldSymbols}{\mathbf{G}}{G}^{#1}(\parameters)}
\newcommand{\cutg}{\ifbool{boldSymbols}{\mathbf{g}}{g}}
\newcommand{\cuth}{h}
\newcommand{\cutu}{\ifbool{boldSymbols}{\mathbf{u}}{u}}
\newcommand{\cutv}{\ifbool{boldSymbols}{\mathbf{v}}{v}}
\newcommand{\disj}{\ifbool{boldSymbols}{\boldsymbol{\pi}}{\pi}}
\newcommand{\disjvalue}{\ifbool{boldSymbols}{\pi_0}{\eta}}
\newcommand{\normalization}{\ifbool{boldSymbols}{\mathbf{D}}{D}}
\newcommand{\lr}{\mu}
\newcommand{\normtype}{p}
\newcommand{\rnn}[1]{f(#1)}
\newcommand{\rnnstate}[1]{\ifbool{boldSymbols}{\mathbf{S_{\rm state}}}{s_{\rm state}}^{#1}}
\newcommand{\algostate}[1][]{\ifbool{boldSymbols}{\mathbf{S}}{s}^{#1}(\parameters)}
\newcommand{\lenalgohistory}{M}
\newcommand{\rnndisj}{\ifbool{boldSymbols}{\boldsymbol{\alpha}}{\alpha}}
\newcommand{\rnnnorm}{\ifbool{boldSymbols}{\boldsymbol{\beta}}{\beta}}
\newcommand{\numcuts}{K}
\newcommand{\numiterations}{R}
\newcommand{\iteration}{r}
\newcommand{\loss}{L(\rnnparameters)}
\newcommand{\trainingset}{\mathcal{T}}
\newcommand{\ve}{\ifbool{boldSymbols}{v}{t}}
\newcommand{\uzero}{\ifbool{boldSymbols}{{u}_0}{u_{\numconstraints+1}}}
\newcommand{\vzero}{\ifbool{boldSymbols}{{v}_0}{v_{\numconstraints+1}}}
\newcommand{\subaddfn}{\Phi}
\newcommand{\doubleu}{\ifbool{boldSymbols}{\mathbf{w}}{w}}
\newcommand{\doubleuplus}{\ifbool{boldSymbols}{\mathbf{w}}{w}_+}
\newcommand{\doubleuminus}{\ifbool{boldSymbols}{\mathbf{w}}{w}_-}
\newcommand{\transpose}{\ifbool{boldSymbols}{\top}{T}}
\newcommand{\gomorydisjpart}{\ifbool{boldSymbols}{\mathbf{m}}{q}}
% for lemmas and stuff
\newcommand{\lemmay}{\ifbool{boldSymbols}{\mathbf{y}}{y}}
\newcommand{\onezerovec}{\ifbool{boldSymbols}{\mathbf{r}}{\xi}}
\newcommand{\utilde}{\tilde{\ifbool{boldSymbols}{\mathbf{u}}{u}}}
\newcommand{\vtilde}{\ifbool{boldSymbols}{\mathbf{v}}{v}}
\newcommand{\spareMone}{\ifbool{boldSymbols}{\mathbf{m}}{q}_1}
\newcommand{\spareMtwo}{\ifbool{boldSymbols}{\mathbf{m}}{q}_2}
\newcommand{\spareMthree}{\ifbool{boldSymbols}{\mathbf{m}}{q}_3}
\newcommand{\spareMfour}{\ifbool{boldSymbols}{\mathbf{m}}{q}_4}
\newcommand{\spareMfive}{\ifbool{boldSymbols}{\mathbf{m}}{q}_5}
\newcommand{\sparescalarone}{m_1}
\newcommand{\sparescalartwo}{m_2}
\newcommand{\ellipse}{\mathcal{E}}
\newcommand{\fractionalpart}[1]{\{ #1 \}}
\newcommand{\zerovec}{\ifbool{boldSymbols}{\mathbf{0}}0}



%Examples
\newcommand{\facilityvars}{\ifbool{boldSymbols}{\mathbf{y}}{y}}
\newcommand{\facilitycosts}{\ifbool{boldSymbols}{\mathbf{c}}{c}(\parameters)}
\newcommand{\facilitytransport}[1]{{e}_{#1}(\parameters)}
\newcommand{\demands}[1]{{d}_{#1}}
\newcommand{\caps}[1]{{C}_{#1}}
\newcommand{\customers}{\mathcal{C}}
\newcommand{\facilities}{\mathcal{F}}

% for the optimal control problem
\newcommand{\controltime}{\tau}
\newcommand{\controlmaxtime}{H}
\newcommand{\power}{P}
\newcommand{\maxpower}{\power^{\text{max}}}
\newcommand{\samplingtime}{\upsilon}
\newcommand{\powerload}{\power^{\text{load}}}
\newcommand{\energy}{E}
\newcommand{\minenergy}{\energy^{\text{min}}}
\newcommand{\maxenergy}{\energy^{\text{max}}}
\newcommand{\initenergy}{\energy^{\text{init}}}
\newcommand{\fuelstate}{\zeta}
\newcommand{\alphacontrol}{\alpha}
\newcommand{\betacontrol}{\omega}
\newcommand{\gammacontrol}{\delta}
\newcommand{\dcontrol}{\xi}
\newcommand{\hcontrol}{h}
\newcommand{\wcontrol}{\psi}
\newcommand{\fuelstateinit}{\fuelstate^{\text{init}}}
\newcommand{\scontrol}{k}
\newcommand{\scontrolinit}{s^{\text{init}}}
\newcommand{\numswitchingsinit}{\numswitchings_{\text{init}}}
\newcommand{\dcontrolpast}{\dcontrol^{\text{past}}}
\newcommand{\nsw}{N^{\text{sw}}}
\newcommand{\Gcontrol}{G}
\newcommand{\controlf}{f}
\newcommand{\dpast}{\dcontrol^{\text{past}}}


==> headers/head.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
% Images and plots
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage[colorlinks,
            linkcolor=BlueViolet,
            citecolor=blue,
            urlcolor=blue,
            bookmarks]{hyperref}
\usepackage{graphicx, pgfplots, subcaption, standalone, pgf, tikz}
\usepackage[justification=centering]{caption}
\usepackage[sort&compress,numbers,sectionbib]{natbib}
\usepackage{comment, url,float, setspace, xspace}
\pgfplotsset{compat=1.17}
\usepackage{array, bm, amssymb, amsfonts,  mathtools, nccmath}
\usepackage[inline]{enumitem}
\renewcommand\arraystretch{1.2}
\setlength{\arraycolsep}{5pt} % reset to default since lncs makes it tiny
\setlist[enumerate]{label=(\roman*.)}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage[nameinlink]{cleveref}
\usepackage{booktabs, longtable, multirow, multicol, adjustbox}	
\newcommand{\todo}[1]{ {\color{Turquoise} #1} }


%ORCIDs
\definecolor{lime}{HTML}{A6CE39}
\DeclareRobustCommand{\orcidicon}{
    \hspace{-3mm}
	\begin{tikzpicture} 
    \draw[lime, fill=lime] (0,0) circle [radius=0.15] node[white] { 
        {\fontfamily{qag}\selectfont \tiny ID} 
    };
	\end{tikzpicture} 
    \hspace{-2mm}
}

\foreach \x in {A, ..., Z}{\expandafter\xdef\csname orcid\x\endcsname{\noexpand\href{https://orcid.org/\csname orcidauthor\x\endcsname}{\noexpand\orcidicon} } }

\raggedbottom

